Report of the Topical Group on Top quark physics and heavy flavor production for Snowmass 2021

This report summarizes the work of the Energy Frontier Topical Group on EW Physics: Heavy flavor and top quark physics (EF03) of the 2021 Community Summer Study (Snowmass). It aims to highlight the physics potential of top-quark studies and heavy-flavor production processes (bottom and charm) at the HL-LHC and possible future hadron and lepton colliders and running scenarios.

==> TOPHF/TOPHF-XS-LHC-exp.tex <==




\FloatBarrier
\subsection{Experimental aspects of \texorpdfstring{$pp \to t\bar t$}{pp to tt}}
\label{sec:TOPHF-XS-LHC-ttexp}
%Author: Regina Demina

Top-quark pair production in hadron machines is interesting to study for several reasons. First, it is the leading source of top quarks, and second, top pair production is one of the main background processes to most searches for new physics. Hence its precise modeling is essential for a reliable extraction of the new physics signal. Third, the top quark itself has a chance to originate from a decay of new particles, e.g. heavy replica of the Higgs boson. Such a process would result in a resonant and interference signal on top of the SM continuum production. And last but not least, it is an important test of  perturbative QCD, which should work well at these high energies, as well as of electroweak (EW) theory. 

The $\ttbar$ cross-section measurements at the Tevatron and the LHC are summarized in Figure~\ref{fig:ttXsecs}. The cross-sections have been measured to better than 5\% uncertainty. The ATLAS+CMS combination at 8~TeV has an uncertainty of only 2.5\%. The largest contributions to this uncertainty are from the luminosity determination and theory modelling of the $\ttbar$ system. Reducing these uncertainties by another factor two should be possible by the end of the HL-LHC~\cite{Azzi:2019yne}, achieving an uncertainty around 1\%.

\begin{figure}[!h!tb]
\centering
\includegraphics[width=0.6\textwidth]{TOPHF/plots/tt_curve_toplhcwg_sep21.pdf}
\caption{Cross-section measurement for $\ttbar$ production at the LHC at different CM energies. From~\cite{LHCtopWG}.}
\label{fig:ttXsecs}
\end{figure}

In the study of top-quark pair production in hadron machines theory and experiment are closely connected, motivating and cross checking each other. For example, the large charge asymmetry in $t\bar{t}$ production observed at the Tevatron~\cite{D0:2007ihv},~\cite{CDF:2008nne} was not explained by the NLO level calculations~\cite{Kuhn:1998kw} leading to a suite of papers suggesting beyond the SM explanations (see e.g. ~\cite{Kamenik:2011wt}). Yet, the inclusion of the EW corrections~\cite{Bernreuther:2012sx} and the extension of the calculations to NNLO~\cite{Czakon:2014xsa} demonstrated a good agreement with a combined result from CDF and D0~\cite{CDF:2017cvy}. 

Similarly, original data from both ATLAS and CMS demonstrated a disagreement in the distribution in the top-quark $p_T$ with the predictions based on NLO simulations. Latest results at the parton level obtained by CMS compared to NNLO level MATRIX simulations~\cite{Grazzini:2017mhc}, \cite{Czakon:2015owf} demonstrated a much better agreement~\cite{CMS:2021vhb} as shown in Figure~\ref{fig:ttXsect}. Similar measurement performed by ATLAS~\cite{ATLAS:2022xfj}  was compared to different simulations with the best agreement demonstrated by POWHEG~\cite{Alioli:2010xd} +PYTHIA8~\cite{Sjostrand:2014zea} reweighted to NNLO prediction~\cite{Czakon:2017wor} with EW corrections.  
\begin{figure}[!h!tb]
\centering
\includegraphics[width=0.45\textwidth]{TOPHF/plots/absxsec_thadpth_log.pdf}
\includegraphics[width=0.54\textwidth]{TOPHF/plots/fig_22a.pdf}
%\includegraphics[width=0.45\textwidth]{CMS-TOP-17-002_Figure_042-e.pdf}
\caption{The normalized
differential cross section of \ttbar\ production as a function of top quark $p_{\mathrm{T}}$
compared to several models at the parton level measured by CMS(left) and ATLAS(right).}
\label{fig:ttXsect}
\end{figure}

The realization that the EW corrections are important in $t\bar{t}$ production resulted in a new method of the evaluation of the top quark Yukawa coupling, $y_t$ using the kinematics of the top and and anti-top quark near the production threshold~\cite{Kuhn:2013zoa}. An example of a Feynman diagram that includes a virtual exchange of EW bosons  including Higgs boson is shown  in the left of Figure~\ref{fig:Yt_theory}.   The interference of such diagram with the tree-level process is proportional $y_t^2$. Hence, increased values of $y_t$ would  result in significant distortions of the distribution in the invariant mass of top and anti-top quarks, as well as the difference in rapidity between the two as shown in Figure~\ref{fig:Yt_theory} (center and right). Comparing data to predictions generated with different values of  $y_t$ allowed CMS to constrain it to be less than $1.67$~\cite{CMS:2019art} in lepton+jets channel and  $1.54$~\cite{CMS:2020djy} in the dilepton channel at the 95\% CL. These results, though not as sensitive as $Y_t$ measurement from a combined analysis of Higgs boson production in gluon fusion and  $t\bar{t}H$ channels, have an advantage of not being dependent on the assumption about the values of the other Higgs boson couplings. The production of four top quarks discussed in Section.~\ref{sec:TOPHF-4top-production} has the same advantage, but so far is not as sensitive. At the same time while the four top quark production process is statistically limited, measurement of $y_t$ from the $t\bar{t}$ kinematics is partially  limited by systematic uncertainties, among which the leading source of theoretical uncertainties are the modeling of parton shower and color reconnection. Future improvements in the $y_t$ measurements require a better understanding of these uncertainties, or development of reliable techniques to constrain them in situ.

\begin{figure}
\centering
\includegraphics[width=0.38\textwidth]{TOPHF/plots/CMS-TOP-17-004_Figure_001-a.pdf} \\
\includegraphics[width=0.48\textwidth]{TOPHF/plots/Fig3_a.pdf}
\includegraphics[width=0.48\textwidth]{TOPHF/plots/Fig3_b.pdf}
\caption{ 
 (Top) An example of Feynman diagrams of \ttbar\ production with virtual exchange of EW  bosons $\Gamma$, including Higgs boson. (Bottom) The dependence of EW corrections to \ttbar\ production for different values of $y_t$ on $M_{\ttbar}$ (left) and $\Delta y_{\ttbar}$ (right), generated by \textsc{hathor}~\cite{Aliev:2010zk}.}
\label{fig:Yt_theory}
\end{figure}

\begin{comment}
Inclusion of non-relativistic QCD effects showed that with a small probability a top-anti-top bound state can form just below the threshold of $t\bar{t}$ production (at about $M_{t\bar{t}}=344$~GeV) ~\cite{Kiyo_2009}, \cite{Fuks:2021xje}. This color singlet state is expected to have quantum numbers of the $\eta$ resonance, and a fairly narrow width $~7$ Gev, as shown in Figure~\ref{fig:toponium} (left). An observation of a toponium signal would be rather spectacular though it is quite challenging given that the experimental  resolution in $t\bar{t}$ invariant mass is about three time larger than the natural width of the resonance and the cross section of its production is rather small (about $6.5$ pb). For illustration in Figure~\ref{fig:toponium} (right) we show the experimentally measured distribution in top-antitop invariant mass. The first bin in this distribution corresponds to the entire region of the predicted spectrum on the left. An improvement in the resolution of the \ttbar\ invariant mass, increased statistics and improved understanding of the systematic uncertainties at the threshold of \ttbar\ production are needed to observe this toponium state. 
\begin{figure}[!h!tb]
\centering
\includegraphics[width=0.51\textwidth]{TOPHF/plots/Singlet_Octet.png}
\includegraphics[width=0.48\textwidth]{TOPHF/plots/CMS-TOP-20-001_Figure_019-a.pdf}
\caption{
(Left) $M_{t\bar{t}}$ distribution for color singlet and color octet \ttbar\ states near the production threshold (plot from ~\cite{Kiyo_2009}). 
(Right)Measured cross section as a function of $M_{t\bar{t}}$.
}
\label{fig:toponium}
\end{figure}

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FloatBarrier
\subsection{Experimental aspects of single top-quark production and \texorpdfstring{$V_{tb}$}{Vtb}}
\label{sec:TOPHF-XS-LHC-stexp}

In the SM, single top-quark production is a charged-current electroweak process that involves the $tWb$ vertex in the production of the top quark and in its decay, with only negligible contributions from $tWd$ and $tWs$ couplings, and even smaller contributions from Flavor-Changing Neutral Currents (FCNC, see Section~\ref{sec:TOPHF-BSM})~\cite{Giammanco:2017xyn}. Precise measurements of single top-quark cross sections are motivated by their sensitivity to new physics that modifies either the production or the decay vertex or both~\cite{AguilarSaavedra:2008zc}. The single top-quark production cross section under the assumption of SM-type left-handed couplings is proportional to the square of the Cabibbo-Kobayashi-Maskawa (CKM)~\cite{Cabibbo:1963yz,Kobayashi:1973fv} matrix element $V_{tb}$~\cite{Alwall:2006bx,Lacker:2012ek}.

\begin{figure}[!h!tb]
\centering
\includegraphics[width=0.8\textwidth]{TOPHF/plots/singletop_allchannels_nov20.pdf}
\caption{Cross-section measurement for single-top quark production at the LHC at different CM energies. From~\cite{LHCtopWG}. }
\label{fig:singletxs}
\end{figure}

The single top cross-section measurements at the LHC are summarized in Figure~\ref{fig:singletxs}. 
The $t$-channel mode has the largest production cross section and smallest uncertainty, 6.6\% in the 8~TeV LHC combination~\cite{atlas:2019hhu}. The largest uncertainties are due to the theory modeling of the single top signal and the $\ttbar$ background. The measurements at 13~TeV in Run~2 have not yet been finalized, and the combination has not been completed. It is expected that the uncertainties will be somewhat smaller due to the improved theory modeling. For the HL-LHC, these uncertainties are projected to be reduced by another factor two, to an uncertainty of about 2\%. However, this requires significant improvements in the modeling of the top-quark final state and parton shower~\cite{QCDreport}.



The sensitivity of single-top quark production to the CKM matrix elements $V_{tu}$, $V_{ts}$ and $V_{tb}$ can be enhanced through measurements of ratios and differential distributions~\cite{Fang:2018lgq}. This study obtains an uncertainty on $V_{tb}$ of about 1\% with 8~TeV data. The  expected sensitivity for $V_{tb}$ at the HL-LHC is about 0.15\%~\cite{Fang:2018lgq}.

At a lepton collider, single top-quark production in the SM occurs through lepton-photon scattering~\cite{Escamilla:2017pvd}, a process that can be observed at collision energies above 0.5~TeV. The CKM matrix element $V_{tb}$ by contrast is included in global EW fits; it is proportional to the left-handed coupling of the top quark to the $W$ boson and $b$ quark. In this way, it can be constrained to significantly better than 1\% in precision $\ttbar$ measurements at lepton colliders, see Ref.~\cite{EWreport}.

==> TOPHF/TOPHF-XS-PDF.tex <==
\FloatBarrier
\subsection{PDF constraints from top-quark observables}

==> TOPHF/TOPHF-XS-ee.tex <==
% Compositeness is relevant at a muon collider and could be covered here. 

%\subsection{$l^+ l^- \to t\bar t, t\bar tV \, (V=\gamma,Z,W^\pm)$, single top, $\ldots$}
%\label{sec:TOPHF-XS-ee}
% This is covered in the top-quark coupling measurements section below.
